A search for gravitational waves associated with the August 2006 timing glitch of the Vela pulsar

The physical mechanisms responsible for pulsar timing glitches are thought to excite quasi-normal mode oscillations in their parent neutron star that couple to gravitational wave emission. In August 2006, a timing glitch was observed in the radio emission of PSR B0833-45, the Vela pulsar. At the time of the glitch, the two co-located Hanford gravitational wave detectors of the Laser Interferometer Gravitational-wave observatory (LIGO) were operational and taking data as part of the fifth LIGO science run (S5). We present the first direct search for the gravitational wave emission associated with oscillations of the fundamental quadrupole mode excited by a pulsar timing glitch. No gravitational wave detection candidate was found. We place Bayesian 90% confidence upper limits of 6.3e-21 to 1.4e-20 on the peak intrinsic strain amplitude of gravitational wave ring-down signals, depending on which spherical harmonic mode is excited. The corresponding range of energy upper limits is 5.0e44 to 1.3e45 erg.

==> authorlist.tex <==
% Based on RevTEX4
%
%
% EXTEND THE SYMBOL LIST FOR FOOTNOTING THE ALTERNATE
%AFFILIATIONS IN THE AUTHOR LIST


\makeatletter
\def\@fnsymbol#1{\ifcase#1\or * \or  $+$ \or  \$ \or \#  \or \dag \or \ddag \or
$\mathsection$ \or $ \mathparagraph$ \or $\|$  \or
\textordfeminine \or \textbullet   \or ** \or $++$ \or  \$\$ \or
\#\#  \or \dag\dag \or \ddag\ddag \or $\mathsection\mathsection$
\or $ \mathparagraph\mathparagraph$ \or $\|\|$  \or
\textordfeminine\textordfeminine \or \textbullet \textbullet \or
*** \or $+++$ \or  \$\$\$ \or \#\#  \or \dag\dag \or \ddag\ddag
\or $\mathsection \mathsection\mathsection$ \or $ \mathparagraph
\mathparagraph\mathparagraph$ \or $\|\|\|$  \or
\textordfeminine\textordfeminine\textordfeminine \or
\textbullet\textbullet\textbullet \or \else \@ctrerr\fi}
%\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\makeatother
%********************* cut here mark*******************
%NOTE ADD altafillletter to \documentclass if lettered affiliation footnotes are desired
% EXAMPLE:
%
%\documentclass[prd,superscriptaddress,showpacs,amssymb,amsmath,amsfonts,aps,altaffilletter]{revtex4}
%
%%%%%%%%%%%% Institutes Number and definitions %%%%%%%%%%%
%
% This list was generated on 5 Nov 2009 A4 DCC LIGO - T0900390-v2

\newcommand*{\AG}{Albert-Einstein-Institut, Max-Planck-Institut f\"{u}r Gravitationsphysik, D-14476 Golm, Germany}
\affiliation{\AG}
\newcommand*{\AH}{Albert-Einstein-Institut, Max-Planck-Institut f\"{u}r Gravitationsphysik, D-30167 Hannover, Germany}
\affiliation{\AH}
\newcommand*{\AU}{Andrews University, Berrien Springs, MI 49104 USA}
\affiliation{\AU}
\newcommand*{\AN}{Australian National University, Canberra, 0200, Australia}
\affiliation{\AN}
\newcommand*{\CH}{California Institute of Technology, Pasadena, CA  91125, USA}
\affiliation{\CH}
\newcommand*{\CA}{Caltech-CaRT, Pasadena, CA  91125, USA}
\affiliation{\CA}
\newcommand*{\CU}{Cardiff University, Cardiff, CF24 3AA, United Kingdom}
\affiliation{\CU}
\newcommand*{\CL}{Carleton College, Northfield, MN  55057, USA}
\affiliation{\CL}
\newcommand*{\CS}{Charles Sturt University, Wagga Wagga, NSW 2678, Australia}
\affiliation{\CS}
\newcommand*{\CO}{Columbia University, New York, NY  10027, USA}
\affiliation{\CO}
\newcommand*{\ER}{Embry-Riddle Aeronautical University, Prescott, AZ   86301 USA}
\affiliation{\ER}
\newcommand*{\EU}{E\"{o}tv\"{o}s University, ELTE 1053 Budapest, Hungary}
\affiliation{\EU}
\newcommand*{\HC}{Hobart and William Smith Colleges, Geneva, NY  14456, USA}
\affiliation{\HC}
\newcommand*{\IA}{Institute of Applied Physics, Nizhny Novgorod, 603950, Russia}
\affiliation{\IA}
\newcommand*{\IU}{Inter-University Centre for Astronomy  and Astrophysics, Pune - 411007, India}
\affiliation{\IU}
\newcommand*{\HU}{Leibniz Universit\"{a}t Hannover, D-30167 Hannover, Germany}
\affiliation{\HU}
\newcommand*{\CT}{LIGO - California Institute of Technology, Pasadena, CA  91125, USA}
\affiliation{\CT}
\newcommand*{\LO}{LIGO - Hanford Observatory, Richland, WA  99352, USA}
\affiliation{\LO}
\newcommand*{\LV}{LIGO - Livingston Observatory, Livingston, LA  70754, USA}
\affiliation{\LV}
\newcommand*{\LM}{LIGO - Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\affiliation{\LM}
\newcommand*{\LU}{Louisiana State University, Baton Rouge, LA  70803, USA}
\affiliation{\LU}
\newcommand*{\LE}{Louisiana Tech University, Ruston, LA  71272, USA}
\affiliation{\LE}
\newcommand*{\MEGA}{McNeese State University, Lake Charles, LA 70609, USA}
\affiliation{\MEGA}
\newcommand*{\MT}{Montana State University, Bozeman, MT 59717, USA}
\affiliation{\MT}
\newcommand*{\MS}{Moscow State University, Moscow, 119992, Russia}
\affiliation{\MS}
\newcommand*{\ND}{NASA/Goddard Space Flight Center, Greenbelt, MD  20771, USA}
\affiliation{\ND}
\newcommand*{\NA}{National Astronomical Observatory of Japan, Tokyo  181-8588, Japan}
\affiliation{\NA}
\newcommand*{\NO}{Northwestern University, Evanston, IL  60208, USA}
\affiliation{\NO}
\newcommand*{\RI}{Rochester Institute of Technology, Rochester, NY  14623, USA}
\affiliation{\RI}
\newcommand*{\RA}{Rutherford Appleton Laboratory, HSIC, Chilton, Didcot, Oxon OX11 0QX United Kingdom}
\affiliation{\RA}
\newcommand*{\SJ}{San Jose State University, San Jose, CA 95192, USA}
\affiliation{\SJ}
\newcommand*{\SM}{Sonoma State University, Rohnert Park, CA 94928, USA}
\affiliation{\SM}
\newcommand*{\SE}{Southeastern Louisiana University, Hammond, LA  70402, USA}
\affiliation{\SE}
\newcommand*{\SO}{Southern University and A\&M College, Baton Rouge, LA  70813, USA}
\affiliation{\SO}
\newcommand*{\SA}{Stanford University, Stanford, CA  94305, USA}
\affiliation{\SA}
\newcommand*{\SR}{Syracuse University, Syracuse, NY  13244, USA}
\affiliation{\SR}
\newcommand*{\PU}{The Pennsylvania State University, University Park, PA  16802, USA}
\affiliation{\PU}
\newcommand*{\UM}{The University of Melbourne, Parkville VIC 3010, Australia}
\affiliation{\UM}
\newcommand*{\MI}{The University of Mississippi, University, MS 38677, USA}
\affiliation{\MI}
\newcommand*{\SF}{The University of Sheffield, Sheffield S10 2TN, United Kingdom}
\affiliation{\SF}
\newcommand*{\TA}{The University of Texas at Austin, Austin, TX 78712, USA}
\affiliation{\TA}
\newcommand*{\TC}{The University of Texas at Brownsville and Texas Southmost College, Brownsville, TX  78520, USA}
\affiliation{\TC}
\newcommand*{\TR}{Trinity University, San Antonio, TX  78212, USA}
\affiliation{\TR}
\newcommand*{\BB}{Universitat de les Illes Balears, E-07122 Palma de Mallorca, Spain}
\affiliation{\BB}
\newcommand*{\UA}{University of Adelaide, Adelaide, SA 5005, Australia}
\affiliation{\UA}
\newcommand*{\BR}{University of Birmingham, Birmingham, B15 2TT, United Kingdom}
\affiliation{\BR}
\newcommand*{\FA}{University of Florida, Gainesville, FL  32611, USA}
\affiliation{\FA}
\newcommand*{\GU}{University of Glasgow, Glasgow, G12 8QQ, United Kingdom}
\affiliation{\GU}
\newcommand*{\MD}{University of Maryland, College Park, MD 20742 USA}
\affiliation{\MD}
\newcommand*{\AM}{University of Massachusetts - Amherst, Amherst, MA 01003, USA}
\affiliation{\AM}
\newcommand*{\MU}{University of Michigan, Ann Arbor, MI  48109, USA}
\affiliation{\MU}
\newcommand*{\MN}{University of Minnesota, Minneapolis, MN 55455, USA}
\affiliation{\MN}
\newcommand*{\OU}{University of Oregon, Eugene, OR  97403, USA}
\affiliation{\OU}
\newcommand*{\RO}{University of Rochester, Rochester, NY  14627, USA}
\affiliation{\RO}
\newcommand*{\SL}{University of Salerno, I-84084 Fisciano (Salerno), Italy and INFN}
\affiliation{\SL}
\newcommand*{\SN}{University of Sannio at Benevento, I-82100 Benevento, Italy and INFN}
\affiliation{\SN}
\newcommand*{\SH}{University of Southampton, Southampton, SO17 1BJ, United Kingdom}
\affiliation{\SH}
\newcommand*{\SC}{University of Strathclyde, Glasgow, G1 1XQ, United Kingdom}
\affiliation{\SC}
\newcommand*{\WA}{University of Western Australia, Crawley, WA 6009, Australia}
\affiliation{\WA}
\newcommand*{\UW}{University of Wisconsin-Milwaukee, Milwaukee, WI  53201, USA}
\affiliation{\UW}
\newcommand*{\WU}{Washington State University, Pullman, WA 99164, USA}
\affiliation{\WU}
\newcommand*{\HartRAOa}{Hartebeesthoek Radio Astronomy Observatory. PO Box 443, Krugersdorp, 1740, South Africa}
\newcommand*{\HartRAOb}{School of Physics, University of the Witwatersrand, Private Bag 3, WITS 2040, South Africa}





\author{J.~Abadie}    \affiliation{\CT}    
\author{B.~P.~Abbott}    \affiliation{\CT}    
\author{R.~Abbott}    \affiliation{\CT}    
\author{R.~Adhikari}    \affiliation{\CT}    
\author{P.~Ajith}    \affiliation{\CT}    
\author{B.~Allen}    \affiliation{\AH}  \affiliation{\UW}  
\author{G.~Allen}    \affiliation{\SA}   
\author{E.~Amador~Ceron}	\affiliation{\UW} 
\author{R.~S.~Amin}    \affiliation{\LU}    
\author{S.~B.~Anderson}    \affiliation{\CT}    
\author{W.~G.~Anderson}    \affiliation{\UW}    
\author{M.~A.~Arain}    \affiliation{\FA}    
\author{M.~Araya}    \affiliation{\CT}        
\author{Y.~Aso}    \affiliation{\CT}    
\author{S.~Aston}    \affiliation{\BR}    
\author{P.~Aufmuth}    \affiliation{\HU}    
\author{C.~Aulbert}    \affiliation{\AH}    
\author{S.~Babak}    \affiliation{\AG}    
\author{P.~Baker}    \affiliation{\MT}    
\author{S.~Ballmer}    \affiliation{\CT}       
\author{D.~Barker}    \affiliation{\LO}    
\author{B.~Barr}    \affiliation{\GU}    
\author{P.~Barriga}    \affiliation{\WA}    
\author{L.~Barsotti}    \affiliation{\LM}    
\author{M.~A.~Barton}    \affiliation{\LO}    
\author{I.~Bartos}    \affiliation{\CO}    
\author{R.~Bassiri}    \affiliation{\GU}    
\author{M.~Bastarrika}    \affiliation{\GU}    
\author{B.~Behnke}    \affiliation{\AG}    
\author{M.~Benacquista}    \affiliation{\TC}    
% ANDREW MELATOS STUDENT
\author{M.~F.~Bennett}		\affiliation{\UM}
\author{J.~Betzwieser}    \affiliation{\CT}    
\author{P.~T.~Beyersdorf}    \affiliation{\SJ}    
\author{I.~A.~Bilenko}    \affiliation{\MS}    
\author{G.~Billingsley}    \affiliation{\CT}    
\author{R.~Biswas}    \affiliation{\UW}    
\author{E.~Black}    \affiliation{\CT}    
\author{J.~K.~Blackburn}    \affiliation{\CT}    
\author{L.~Blackburn}    \affiliation{\LM}    
\author{D.~Blair}    \affiliation{\WA}    
\author{B.~Bland}    \affiliation{\LO} 
\author{O.~Bock}	\affiliation{\AH}   
\author{T.~P.~Bodiya}    \affiliation{\LM}    
\author{R.~Bondarescu}    \affiliation{\PU}    
\author{R.~Bork}    \affiliation{\CT}    
\author{M.~Born}    \affiliation{\AH}    
\author{S.~Bose}    \affiliation{\WU}    
\author{P.~R.~Brady}    \affiliation{\UW}    
\author{V.~B.~Braginsky}    \affiliation{\MS}    
\author{J.~E.~Brau}    \affiliation{\OU} 
\author{J.~Breyer}	\affiliation{\AH}   
\author{D.~O.~Bridges}    \affiliation{\LV}    
\author{M.~Brinkmann}    \affiliation{\AH}  
\author{M.~Britzger}	\affiliation{\AH}  
\author{A.~F.~Brooks}    \affiliation{\CT}    
\author{D.~A.~Brown}    \affiliation{\SR}          
\author{A.~Bullington}    \affiliation{\SA}    
\author{A.~Buonanno}    \affiliation{\MD}    
\author{O.~Burmeister}    \affiliation{\AH}    
\author{R.~L.~Byer}    \affiliation{\SA}    
\author{L.~Cadonati}    \affiliation{\AM}  
\author{J.~Cain}		\affiliation{\MI}  
\author{J.~B.~Camp}    \affiliation{\ND}    
\author{J.~Cannizzo}    \affiliation{\ND}    
\author{K.~C.~Cannon}    \affiliation{\CT}    
\author{J.~Cao}    \affiliation{\LM}  
\author{C.~Capano}	\affiliation{\SR}  
\author{L.~Cardenas}    \affiliation{\CT}       
\author{S.~Caudill}    \affiliation{\LU}    
\author{M.~Cavagli\`{a}}    \affiliation{\MI}    
\author{C.~Cepeda}    \affiliation{\CT}    
\author{T.~Chalermsongsak}    \affiliation{\CT}    
\author{E.~Chalkley}    \affiliation{\GU}    
\author{P.~Charlton}    \affiliation{\CS}    
\author{S.~Chatterji}    \affiliation{\CT}    
\author{S.~Chelkowski}    \affiliation{\BR}    
\author{Y.~Chen}    \affiliation{\CA}  
\author{N.~Christensen}    \affiliation{\CL}
\author{S.~S.~Y.~Chua}		\affiliation{\AN}    
\author{C.~T.~Y.~Chung}    \affiliation{\UM}    
\author{D.~Clark}    \affiliation{\SA}    
\author{J.~Clark}    \affiliation{\CU}    
\author{J.~H.~Clayton}    \affiliation{\UW}        
\author{R.~Conte}    \affiliation{\SL}    
\author{D.~Cook}    \affiliation{\LO}    
\author{T.~R.~C.~Corbitt}    \affiliation{\LM}    
\author{N.~Cornish}    \affiliation{\MT}    
\author{D.~Coward}    \affiliation{\WA}    
\author{D.~C.~Coyne}    \affiliation{\CT}    
\author{J.~D.~E.~Creighton}    \affiliation{\UW}    
\author{T.~D.~Creighton}    \affiliation{\TC}    
\author{A.~M.~Cruise}    \affiliation{\BR}    
\author{R.~M.~Culter}    \affiliation{\BR}    
\author{A.~Cumming}    \affiliation{\GU}    
\author{L.~Cunningham}    \affiliation{\GU} 
\author{K.~Dahl}		\affiliation{\AH}   
\author{S.~L.~Danilishin}    \affiliation{\MS}    
\author{K.~Danzmann}    \affiliation{\AH}  \affiliation{\HU}  
\author{B.~Daudert}    \affiliation{\CT}    
\author{G.~Davies}    \affiliation{\CU}    
\author{E.~J.~Daw}    \affiliation{\SF} 
\author{T.~Dayanga}		\affiliation{\WU}   
\author{D.~DeBra}    \affiliation{\SA}    
\author{J.~Degallaix}    \affiliation{\AH}    
\author{V.~Dergachev}    \affiliation{\MU}        
\author{R.~DeSalvo}    \affiliation{\CT}    
\author{S.~Dhurandhar}    \affiliation{\IU}    
\author{M.~D\'{i}az}    \affiliation{\TC}        
\author{F.~Donovan}    \affiliation{\LM}    
\author{K.~L.~Dooley}    \affiliation{\FA}    
\author{E.~E.~Doomes}    \affiliation{\SO}    
\author{R.~W.~P.~Drever}    \affiliation{\CH} 
\author{J.~Driggers}	\affiliation{\CT}   
\author{J.~Dueck}    \affiliation{\AH}    
\author{I.~Duke}    \affiliation{\LM}    
\author{J.~-C.~Dumas}    \affiliation{\WA}            
\author{M.~Edgar}    \affiliation{\GU}  
\author{M.~Edwards}		\affiliation{\CU}  
\author{A.~Effler}    \affiliation{\LO}    
\author{P.~Ehrens}    \affiliation{\CT}       
\author{T.~Etzel}    \affiliation{\CT}    
\author{M.~Evans}    \affiliation{\LM}    
\author{T.~Evans}    \affiliation{\LV}    
\author{S.~Fairhurst}    \affiliation{\CU}    
\author{Y.~Faltas}    \affiliation{\FA}    
\author{Y.~Fan}    \affiliation{\WA}    
\author{D.~Fazi}    \affiliation{\CT}    
\author{H.~Fehrmann}    \affiliation{\AH}    
\author{L.~S.~Finn}    \affiliation{\PU}    
\author{K.~Flasch}    \affiliation{\UW}    
\author{S.~Foley}    \affiliation{\LM}    
\author{C.~Forrest}    \affiliation{\RO}    
\author{N.~Fotopoulos}    \affiliation{\UW}       
\author{M.~Frede}    \affiliation{\AH}    
\author{M.~Frei}    \affiliation{\TA}    
\author{Z.~Frei}    \affiliation{\EU}    
\author{A.~Freise}    \affiliation{\BR}    
\author{R.~Frey}    \affiliation{\OU}    
\author{T.~T.~Fricke}    \affiliation{\LU}  
\author{D.~Friedrich}	\affiliation{\AH}  
\author{P.~Fritschel}    \affiliation{\LM}    
\author{V.~V.~Frolov}    \affiliation{\LV}
\author{P.~Fulda}		\affiliation{\BR}    
\author{M.~Fyffe}    \affiliation{\LV}        
\author{J.~A.~Garofoli}    \affiliation{\SR}    
\author{S.~Ghosh}    \affiliation{\WU}    
\author{J.~A.~Giaime}    \affiliation{\LU}  \affiliation{\LV} 
\author{S.~Giampanis}	\affiliation{\AH} 
\author{K.~D.~Giardina}    \affiliation{\LV}       
\author{E.~Goetz}    \affiliation{\MU}    
\author{L.~M.~Goggin}    \affiliation{\UW}    
\author{G.~Gonz\'alez}    \affiliation{\LU}      
\author{S.~Go\ss{}ler}    \affiliation{\AH}        
\author{A.~Grant}    \affiliation{\GU}    
\author{S.~Gras}    \affiliation{\WA}    
\author{C.~Gray}    \affiliation{\LO}        
\author{R.~J.~S.~Greenhalgh}    \affiliation{\RA}    
\author{A.~M.~Gretarsson}    \affiliation{\ER}       
\author{R.~Grosso}    \affiliation{\TC}    
\author{H.~Grote}    \affiliation{\AH}    
\author{S.~Grunewald}    \affiliation{\AG}        
\author{E.~K.~Gustafson}    \affiliation{\CT}    
\author{R.~Gustafson}    \affiliation{\MU}    
\author{B.~Hage}    \affiliation{\HU}    
\author{J.~M.~Hallam}    \affiliation{\BR}    
\author{D.~Hammer}    \affiliation{\UW}    
\author{G.~D.~Hammond}    \affiliation{\GU}    
\author{C.~Hanna}    \affiliation{\CT}    
\author{J.~Hanson}    \affiliation{\LV}    
\author{J.~Harms}    \affiliation{\MN}    
\author{G.~M.~Harry}    \affiliation{\LM}    
\author{I.~W.~Harry}    \affiliation{\CU}    
\author{E.~D.~Harstad}    \affiliation{\OU}    
\author{K.~Haughian}    \affiliation{\GU}    
\author{K.~Hayama}    \affiliation{\AH}
\author{T.~Hayler}		\affiliation{\RA}    
\author{J.~Heefner}    \affiliation{\CT}    
\author{I.~S.~Heng}    \affiliation{\GU}    
\author{A.~Heptonstall}    \affiliation{\CT}    
\author{M.~Hewitson}    \affiliation{\AH}    
\author{S.~Hild}    \affiliation{\BR}    
\author{E.~Hirose}    \affiliation{\SR}    
\author{D.~Hoak}    \affiliation{\LV}    
\author{K.~A.~Hodge}    \affiliation{\CT}    
\author{K.~Holt}    \affiliation{\LV}    
\author{D.~J.~Hosken}    \affiliation{\UA}    
\author{J.~Hough}    \affiliation{\GU}  
\author{E.~Howell}	\affiliation{\WA}  
\author{D.~Hoyland}    \affiliation{\BR}    
\author{B.~Hughey}    \affiliation{\LM}  
\author{S.~Husa}	\affiliation{\BB}  
\author{S.~H.~Huttner}    \affiliation{\GU}    
\author{D.~R.~Ingram}    \affiliation{\LO}    
\author{T.~Isogai}    \affiliation{\CL}        
\author{A.~Ivanov}    \affiliation{\CT}        
\author{W.~W.~Johnson}    \affiliation{\LU}    
\author{D.~I.~Jones}    \affiliation{\SH}    
\author{G.~Jones}    \affiliation{\CU}    
\author{R.~Jones}    \affiliation{\GU}    
\author{L.~Ju}    \affiliation{\WA}    
\author{P.~Kalmus}    \affiliation{\CT}    
\author{V.~Kalogera}    \affiliation{\NO}    
\author{S.~Kandhasamy}    \affiliation{\MN}    
\author{J.~Kanner}    \affiliation{\MD}        
\author{E.~Katsavounidis}    \affiliation{\LM}    
\author{K.~Kawabe}    \affiliation{\LO}    
\author{S.~Kawamura}    \affiliation{\NA}    
\author{F.~Kawazoe}    \affiliation{\AH}    
\author{W.~Kells}    \affiliation{\CT}    
\author{D.~G.~Keppel}    \affiliation{\CT}    
\author{A.~Khalaidovski}    \affiliation{\AH}    
\author{F.~Y.~Khalili}    \affiliation{\MS}    
\author{R.~Khan}    \affiliation{\CO}    
\author{E.~Khazanov}    \affiliation{\IA}  
\author{H.~Kim}		\affiliation{\AH}  
\author{P.~J.~King}    \affiliation{\CT}    
\author{J.~S.~Kissel}    \affiliation{\LU}    
\author{S.~Klimenko}    \affiliation{\FA}    
\author{K.~Kokeyama}    \affiliation{\NA}    
\author{V.~Kondrashov}    \affiliation{\CT}    
\author{R.~Kopparapu}    \affiliation{\PU}    
\author{S.~Koranda}    \affiliation{\UW}    
\author{D.~Kozak}    \affiliation{\CT}   
\author{V.~Kringel}		\affiliation{\AH} 
\author{B.~Krishnan}    \affiliation{\AG}  
\author{G.~Kuehn}		\affiliation{\AH}
\author{J.~Kullman}		\affiliation{\AH}  
\author{R.~Kumar}    \affiliation{\GU}    
\author{P.~Kwee}    \affiliation{\HU}    
\author{P.~K.~Lam}    \affiliation{\AN}    
\author{M.~Landry}    \affiliation{\LO}
\author{M.~Lang}	\affiliation{\PU}    
\author{B.~Lantz}    \affiliation{\SA} 
\author{N.~Lastzka}		\affiliation{\AH}   
\author{A.~Lazzarini}    \affiliation{\CT}  
\author{P.~Leaci}		\affiliation{\AH}      
\author{M.~Lei}    \affiliation{\CT}    
\author{N.~Leindecker}    \affiliation{\SA}    
\author{I.~Leonor}    \affiliation{\OU}       
\author{H.~Lin}    \affiliation{\FA}    
\author{P.~E.~Lindquist}    \affiliation{\CT}    
\author{T.~B.~Littenberg}    \affiliation{\MT}    
\author{N.~A.~Lockerbie}    \affiliation{\SC}    
\author{D.~Lodhia}    \affiliation{\BR}        
\author{M.~Lormand}    \affiliation{\LV}    
\author{P.~Lu}    \affiliation{\SA}    
\author{M.~Lubinski}    \affiliation{\LO}    
\author{A.~Lucianetti}    \affiliation{\FA}    
\author{H.~L\"{u}ck}    \affiliation{\AH}  \affiliation{\HU} 
\author{A.~Lundgren}	\affiliation{\SR} 
\author{B.~Machenschalk}    \affiliation{\AH}    
\author{M.~MacInnis}    \affiliation{\LM}    
\author{M.~Mageswaran}    \affiliation{\CT}    
\author{K.~Mailand}    \affiliation{\CT}  
\author{C.~Mak}		\affiliation{\CT}  
\author{I.~Mandel}    \affiliation{\NO}    
\author{V.~Mandic}    \affiliation{\MN}    
\author{S.~M\'{a}rka}    \affiliation{\CO}    
\author{Z.~M\'{a}rka}    \affiliation{\CO}    
\author{A.~Markosyan}    \affiliation{\SA}    
\author{J.~Markowitz}    \affiliation{\LM}    
\author{E.~Maros}    \affiliation{\CT}    
\author{I.~W.~Martin}    \affiliation{\GU}    
\author{R.~M.~Martin}    \affiliation{\FA}    
\author{J.~N.~Marx}    \affiliation{\CT}    
\author{K.~Mason}    \affiliation{\LM}    
\author{F.~Matichard}    \affiliation{\LM} \affiliation{\LU}    
\author{L.~Matone}    \affiliation{\CO}    
\author{R.~A.~Matzner}    \affiliation{\TA}    
\author{N.~Mavalvala}    \affiliation{\LM}    
\author{R.~McCarthy}    \affiliation{\LO}    
\author{D.~E.~McClelland}    \affiliation{\AN}    
\author{S.~C.~McGuire}    \affiliation{\SO}        
\author{G.~McIntyre}    \affiliation{\CT}    
\author{D.~J.~A.~McKechan}    \affiliation{\CU}        
\author{M.~Mehmet}    \affiliation{\AH}    
\author{A.~Melatos}    \affiliation{\UM}    
\author{A.~C.~Melissinos}    \affiliation{\RO}    
\author{G.~Mendell}    \affiliation{\LO}   
\author{D.~F.~Men\'{e}ndez}    \affiliation{\PU} 
\author{R.~A.~Mercer}    \affiliation{\UW}
\author{L.~Merrill}		\affiliation{\WA}    
\author{S.~Meshkov}    \affiliation{\CT}    
\author{C.~Messenger}    \affiliation{\AH}    
\author{M.~S.~Meyer}    \affiliation{\LV} 
\author{H.~Miao}		\affiliation{\WA}   
\author{J.~Miller}    \affiliation{\GU}    
\author{Y.~Mino}    \affiliation{\CA}
\author{S.~Mitra}	\affiliation{\CT}    
\author{V.~P.~Mitrofanov}    \affiliation{\MS}    
\author{G.~Mitselmakher}    \affiliation{\FA}    
\author{R.~Mittleman}    \affiliation{\LM}    
\author{O.~Miyakawa}    \affiliation{\CT}    
\author{B.~Moe}    \affiliation{\UW}    
\author{S.~D.~Mohanty}    \affiliation{\TC}    
\author{S.~R.~P.~Mohapatra}    \affiliation{\AM}    
\author{G.~Moreno}    \affiliation{\LO}       
\author{K.~Mors}    \affiliation{\AH}    
\author{K.~Mossavi}    \affiliation{\AH}    
\author{C.~MowLowry}    \affiliation{\AN}    
\author{G.~Mueller}    \affiliation{\FA}    
\author{H.~M\"{u}ller-Ebhardt}    \affiliation{\AH}       
\author{S.~Mukherjee}    \affiliation{\TC}       
\author{A.~Mullavey}    \affiliation{\AN}    
\author{J.~Munch}    \affiliation{\UA}    
\author{P.~G.~Murray}    \affiliation{\GU}        
\author{T.~Nash}    \affiliation{\CT}  
\author{R.~Nawrodt}	\affiliation{\GU}  
\author{J.~Nelson}    \affiliation{\GU}    
\author{G.~Newton}    \affiliation{\GU}    
\author{E.~Nishida}		\affiliation{\NA}
\author{A.~Nishizawa}    \affiliation{\NA}        
\author{J.~O'Dell}    \affiliation{\RA}    
\author{B.~O'Reilly}    \affiliation{\LV}    
\author{R.~O'Shaughnessy}    \affiliation{\PU}    
\author{E.~Ochsner}    \affiliation{\MD}    
\author{G.~H.~Ogin}    \affiliation{\CT} 
\author{R.~Oldenburg}	\affiliation{\UW}   
\author{D.~J.~Ottaway}    \affiliation{\UA}    
\author{R.~S.~Ottens}    \affiliation{\FA}    
\author{H.~Overmier}    \affiliation{\LV}    
\author{B.~J.~Owen}    \affiliation{\PU}
\author{A.~Page}		\affiliation{\BR}    
\author{Y.~Pan}    \affiliation{\MD}    
\author{C.~Pankow}    \affiliation{\FA}    
\author{M.~A.~Papa}    \affiliation{\AG}  \affiliation{\UW}     
\author{P.~Patel}    \affiliation{\CT}   
\author{D.~Pathak}	\affiliation{\CU} 
\author{M.~Pedraza}    \affiliation{\CT}  
\author{L.~Pekowsky}	\affiliation{\SR}  
\author{S.~Penn}    \affiliation{\HC}    
\author{C.~Peralta}		\affiliation{\AG}
\author{A.~Perreca}    \affiliation{\BR}  
\author{M.~Pickenpack}	\affiliation{\AH}    
\author{I.~M.~Pinto}    \affiliation{\SN}    
\author{M.~Pitkin}    \affiliation{\GU}    
\author{H.~J.~Pletsch}    \affiliation{\AH}    
\author{M.~V.~Plissi}    \affiliation{\GU}    
\author{F.~Postiglione}    \affiliation{\SN}    
\author{M.~Principe}    \affiliation{\SN}    
\author{R.~Prix}    \affiliation{\AH}    
\author{L.~Prokhorov}    \affiliation{\MS}    
\author{O.~Puncken}    \affiliation{\AH}    
\author{V.~Quetschke}    \affiliation{\TC}    
\author{F.~J.~Raab}    \affiliation{\LO}    
\author{D.~S.~Rabeling}    \affiliation{\AN}    
\author{H.~Radkins}    \affiliation{\LO}    
\author{P.~Raffai}    \affiliation{\EU}    
\author{Z.~Raics}    \affiliation{\CO}        
\author{M.~Rakhmanov}    \affiliation{\TC}    
\author{V.~Raymond}    \affiliation{\NO}    
\author{C.~M.~Reed}    \affiliation{\LO}    
\author{T.~Reed}    \affiliation{\LE}    
\author{H.~Rehbein}    \affiliation{\AH}    
\author{S.~Reid}    \affiliation{\GU}    
\author{D.~H.~Reitze}    \affiliation{\FA}    
\author{R.~Riesen}    \affiliation{\LV}    
\author{K.~Riles}    \affiliation{\MU}       
\author{P.~Roberts}    \affiliation{\AU}    
\author{N.~A.~Robertson}    \affiliation{\CT}  \affiliation{\GU}  
\author{C.~Robinson}    \affiliation{\CU}    
\author{E.~L.~Robinson}    \affiliation{\AG}    
\author{S.~Roddy}    \affiliation{\LV}    
\author{C.~R\"{o}ver}    \affiliation{\AH}    
\author{J.~Rollins}    \affiliation{\CO}    
\author{J.~D.~Romano}    \affiliation{\TC}    
\author{J.~H.~Romie}    \affiliation{\LV}    
\author{S.~Rowan}    \affiliation{\GU}    
\author{A.~R\"udiger}    \affiliation{\AH}        
\author{K.~Ryan}    \affiliation{\LO}    
\author{S.~Sakata}    \affiliation{\NA}  
\author{L.~Sammut}		\affiliation{\UM}  
\author{L.~Sancho~de~la~Jordana}    \affiliation{\BB}    
\author{V.~Sandberg}    \affiliation{\LO}    
\author{V.~Sannibale}    \affiliation{\CT}    
\author{L.~Santamar\'{i}a}    \affiliation{\AG} 
\author{G.~Santostasi}		\affiliation{\MEGA}   
\author{S.~Saraf}    \affiliation{\SM}  
\author{P.~Sarin}	\affiliation{\LM}      
\author{B.~S.~Sathyaprakash}    \affiliation{\CU}    
\author{S.~Sato}    \affiliation{\NA}    
\author{M.~Satterthwaite}    \affiliation{\AN}    
\author{P.~R.~Saulson}    \affiliation{\SR}    
\author{R.~Savage}    \affiliation{\LO}       
\author{R.~Schilling}    \affiliation{\AH}   
\author{R.~Schnabel}    \affiliation{\AH}    
\author{R.~Schofield}    \affiliation{\OU}    
\author{B.~Schulz}    \affiliation{\AH}    
\author{B.~F.~Schutz}    \affiliation{\AG}  \affiliation{\CU}  
\author{P.~Schwinberg}    \affiliation{\LO}    
\author{J.~Scott}    \affiliation{\GU}    
\author{S.~M.~Scott}    \affiliation{\AN}    
\author{A.~C.~Searle}    \affiliation{\CT}        
\author{F.~Seifert}    \affiliation{\AH}  	\affiliation{\CT}  
\author{D.~Sellers}    \affiliation{\LV}    
\author{A.~S.~Sengupta}    \affiliation{\CT}    
\author{A.~Sergeev}    \affiliation{\IA}    
\author{B.~Shapiro}    \affiliation{\LM}    
\author{P.~Shawhan}    \affiliation{\MD}    
\author{D.~H.~Shoemaker}    \affiliation{\LM}    
\author{A.~Sibley}    \affiliation{\LV}    
\author{X.~Siemens}    \affiliation{\UW}    
\author{D.~Sigg}    \affiliation{\LO}       
\author{A.~M.~Sintes}    \affiliation{\BB} 
\author{G.~Skelton}		\affiliation{\UW}   
\author{B.~J.~J.~Slagmolen}    \affiliation{\AN}    
\author{J.~Slutsky}    \affiliation{\LU}    
\author{J.~R.~Smith}    \affiliation{\SR}    
\author{M.~R.~Smith}    \affiliation{\CT}    
\author{N.~D.~Smith}    \affiliation{\LM}    
\author{K.~Somiya}    \affiliation{\CA}    
\author{B.~Sorazu}    \affiliation{\GU}    
% FIONA
\author{F.~Speirits} \affiliation{\GU}
\author{A.~J.~Stein}    \affiliation{\LM}    
\author{L.~C.~Stein}    \affiliation{\LM}    
\author{S.~Steplewski}    \affiliation{\WU}    
\author{A.~Stochino}    \affiliation{\CT}    
\author{R.~Stone}    \affiliation{\TC}    
\author{K.~A.~Strain}    \affiliation{\GU}    
\author{S.~Strigin}    \affiliation{\MS}    
\author{A.~Stroeer}    \affiliation{\ND}    
\author{A.~L.~Stuver}    \affiliation{\LV}    
\author{T.~Z.~Summerscales}    \affiliation{\AU}        
\author{M.~Sung}    \affiliation{\LU} 
\author{S.~Susmithan}	\affiliation{\WA}   
\author{P.~J.~Sutton}    \affiliation{\CU}    
\author{G.~P.~Szokoly}    \affiliation{\EU}    
\author{D.~Talukder}    \affiliation{\WU}        
\author{D.~B.~Tanner}    \affiliation{\FA}    
\author{S.~P.~Tarabrin}    \affiliation{\MS}    
\author{J.~R.~Taylor}    \affiliation{\AH}    
\author{R.~Taylor}    \affiliation{\CT}        
\author{K.~A.~Thorne}    \affiliation{\LV}
\author{K.~S.~Thorne}	\affiliation{\CA}   
\author{A.~Th\"{u}ring}    \affiliation{\HU} 
\author{C.~Titsler}		\affiliation{\PU}   
\author{K.~V.~Tokmakov}    \affiliation{\GU} 	\affiliation{\SC}   
\author{C.~Torres}    \affiliation{\LV}    
\author{C.~I.~Torrie}    \affiliation{\CT}    \affiliation{\GU}
\author{G.~Traylor}    \affiliation{\LV}    
\author{M.~Trias}    \affiliation{\BB}  
\author{L.~Turner}	\affiliation{\CT}  
\author{D.~Ugolini}    \affiliation{\TR}        
\author{K.~Urbanek}    \affiliation{\SA}    
\author{H.~Vahlbruch}    \affiliation{\HU}    
\author{M.~Vallisneri}    \affiliation{\CA}    
\author{C.~Van~Den~Broeck}    \affiliation{\CU}    
\author{M.~V.~van~der~Sluys}    \affiliation{\NO}    
\author{A.~A.~van~Veggel}    \affiliation{\GU}    
\author{S.~Vass}    \affiliation{\CT}    
\author{R.~Vaulin}    \affiliation{\UW}    
\author{A.~Vecchio}    \affiliation{\BR}    
\author{J.~Veitch}    \affiliation{\BR}    
\author{P.~J.~Veitch}    \affiliation{\UA}    
\author{C.~Veltkamp}    \affiliation{\AH}    
\author{A.~Villar}    \affiliation{\CT}    
\author{C.~Vorvick}    \affiliation{\LO}    
\author{S.~P.~Vyachanin}    \affiliation{\MS}    
\author{S.~J.~Waldman}    \affiliation{\LM}    
\author{L.~Wallace}    \affiliation{\CT}    
\author{A.~Wanner}		\affiliation{\AH}
\author{R.~L.~Ward}    \affiliation{\CT}     
\author{P.~Wei}		\affiliation{\SR}  
\author{M.~Weinert}    \affiliation{\AH}    
\author{A.~J.~Weinstein}    \affiliation{\CT}    
\author{R.~Weiss}    \affiliation{\LM}    
\author{L.~Wen}     \affiliation{\WA}  \affiliation{\CA}
\author{S.~Wen}    \affiliation{\LU}
\author{P.~Wessels}	\affiliation{\AH}    
\author{M.~West}	\affiliation{\SR}
\author{T.~Westphal}	\affiliation{\AH}
\author{K.~Wette}    \affiliation{\AN}    
\author{J.~T.~Whelan}    \affiliation{\RI}  
\author{S.~E.~Whitcomb}    \affiliation{\CT}    
\author{B.~F.~Whiting}    \affiliation{\FA}    
\author{C.~Wilkinson}    \affiliation{\LO}    
\author{P.~A.~Willems}    \affiliation{\CT}    
\author{H.~R.~Williams}    \affiliation{\PU}    
\author{L.~Williams}    \affiliation{\FA}    
\author{B.~Willke}    \affiliation{\AH}  \affiliation{\HU}  
\author{I.~Wilmut}    \affiliation{\RA}    
\author{L.~Winkelmann}    \affiliation{\AH}    
\author{W.~Winkler}    \affiliation{\AH}    
\author{C.~C.~Wipf}    \affiliation{\LM}    
\author{A.~G.~Wiseman}    \affiliation{\UW}    
\author{G.~Woan}    \affiliation{\GU}    
\author{R.~Wooley}    \affiliation{\LV}    
\author{J.~Worden}    \affiliation{\LO}       
\author{I.~Yakushin}    \affiliation{\LV}    
\author{H.~Yamamoto}    \affiliation{\CT} 
\author{K.~Yamamoto}	\affiliation{\AH}   
\author{D.~Yeaton-Massey}    \affiliation{\CT}    
\author{S.~Yoshida}    \affiliation{\SE}    
\author{M.~Zanolin}    \affiliation{\ER}       
\author{L.~Zhang}    \affiliation{\CT} 
\author{Z.~Zhang}	\affiliation{\WA}   
\author{C.~Zhao}    \affiliation{\WA}    
\author{N.~Zotov}    \affiliation{\LE}    
\author{M.~E.~Zucker}    \affiliation{\LM}    
\author{J.~Zweizig}    \affiliation{\CT}    
%
 \collaboration{The LIGO Scientific Collaboration, http://www.ligo.org}
 \noaffiliation
 \author{S.~Buchner} \affiliation{\HartRAOa}  \affiliation{\HartRAOb}

